Unraveling Normal Anatomy via Fluid-Driven Anomaly Randomization

Data-driven machine learning has made significant strides in medical image analysis. However, most existing methods are tailored to specific modalities and assume a particular resolution (often isotropic). This limits their generalizability in clinical settings, where variations in scan appearance arise from differences in sequence parameters, resolution, and orientation. Furthermore, most general-purpose models are designed for healthy subjects and suffer from performance degradation when pathology is present. We introduce UNA (Unraveling Normal Anatomy), the first modality-agnostic learning approach for normal brain anatomy reconstruction that can handle both healthy scans and cases with pathology. We propose a fluid-driven anomaly randomization method that generates an unlimited number of realistic pathology profiles on-the-fly. UNA is trained on a combination of synthetic and real data, and can be applied directly to real images with potential pathology without the need for fine-tuning. We demonstrate UNA's effectiveness in reconstructing healthy brain anatomy and showcase its direct application to anomaly detection, using both simulated and real images from 3D healthy and stroke datasets, including CT and MRI scans. By bridging the gap between healthy and diseased images, UNA enables the use of general-purpose models on diseased images, opening up new opportunities for large-scale analysis of uncurated clinical images in the presence of pathology. Code is available at https://github.com/peirong26/UNA.

==> sec/method/fig/fw_gen.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\resizebox{\textwidth}{!}{
	
	\begin{tikzpicture}[lattice/.cd,spacing/.initial=4,superlattice
  period/.initial=12,amplitude/.initial=2]
	\pgfmathsetmacro{\cubex}{0.29*3}
	\pgfmathsetmacro{\cubey}{0.29*3}
	\pgfmathsetmacro{\cubez}{0.028*3}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	
	%\pgfmathsetmacro{\shift}{0.3}
	%\foreach \i in {-1.15}
	%{
	%\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift+0.1*3,0.15*3,0.1*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	%\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift+0.1*3,0.15*3,0.1*3) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
	%\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift+0.1*3,0.15*3,0.1*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;
	%} 
	%\node at (-1.15+\shift+0.2975*3, 0.3475*3, 0.99*3) {\includegraphics[width=0.104\textwidth]{fig/gen/label.png}};

 
	\pgfmathsetmacro{\shift}{-2.5}
	\foreach \i in {1.3}
	{
	\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift+0.4*3,0.5*3,0.5*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift+0.4*3,0.5*3,0.5*3) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift+0.4*3,0.5*3,0.5*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;
	\node at (\i+\shift+0.409*3, 0.509*3, 0.9*3) {\includegraphics[width=0.104\textwidth]{fig/gen/isles0127_label.png}};
	\node at (\i+\shift+0.409*3, 0.95, 0.9*3) {\tiny $L$};
	}
 
	\foreach \i in {1.995}
	{
	\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift-0.07*3,-0.17*3,-0.12*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.07*3, -0.17*3,-0.12*3) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.07*3,-0.17*3,-0.12*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;	
	\node at (\i+\shift-0.75, -0.35*3, -0.212*3) {\includegraphics[width=0.104\textwidth]{fig/gen/isles0127_patholprob.png}}; 
	\node at (\i+\shift-0.75, -1.64, -0.212*3) {\tiny $P$~(\cref{eq: prob})};
	}


 
	\pgfmathsetmacro{\shift}{0.5}
	\draw[-latex] (-1.15+0.6+\shift, 0.05, 0.25*3) -- (0.1+0.8+\shift, 0.05, 0.25*3); 
	\node at (-1.0+1.15+\shift, -0.11, 0.25*3) {\tiny \text{Deformation}};

 
	\node at (-1.0+1.15+\shift, -0.55, 0.25*3) {\includegraphics[width=0.08\textwidth]{fig/gen/colorbar.png}}; 
	\node at (-1.0+1.15-0.62+\shift, -0.55, 0.25*3) {\tiny \text{0}}; 
	\node at (-1.0+1.15+0.62+\shift, -0.55, 0.25*3) {\tiny \text{1}}; 
	\node at (-1.0+1.15+\shift, -0.8, 0.25*3) {\tiny \text{Anomaly Prob}};

 
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\pgfmathsetmacro{\shift}{0.3}
	\pgfmathsetmacro{\dx}{-5.5}
	\pgfmathsetmacro{\dy}{2.7}
	%\draw[dotted, color = orange!80, line width=0.4mm] (5+\dx+\shift, -4+\dy) -- (6+\dx+\shift, -4+\dy) -- (6+\dx+\shift, -3.3+\dy) -- (5+\dx+\shift, -3.3+\dy) -- (5+\dx+\shift, -4+\dy); 
        
        \begin{scope}[xshift=-5]
            \pgftransformnonlinear{\latticetilt}
            \draw[orange!80,step=0.08,thin] (0.15,0.15) grid (0.88,0.88);
            \draw[->, black] (0.15,0.15) -- +(0.85,0);
            \draw[->, black] (0.15,0.15) -- +(0,0.85);
        \end{scope} 
    
	\draw[->, line width = 0.2mm, color=orange!80] (5.6+\dx+\shift, -2.55+\dy) -- (5.6+\dx+\shift, -2.87+\dy);
 
	\node at (5.45+\dx+\shift, -2.7+\dy) {\tiny $\phi$}; 
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	%\draw[->, line width = 0.2mm, color=matcha!200] (5.5+\dx+\shift, -3.28+\dy) -- (5.5+\dx+\shift, -2.98+\dy);

	\foreach \i in {1.305}
	{
	\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift+0.4*3,0.5*3,0.5*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift+0.4*3,0.5*3,0.5*3) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift+0.4*3,0.5*3,0.5*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;
	\node at (\i+\shift+0.409*3, 0.509*3, 0.9*3) {\includegraphics[width=0.104\textwidth]{fig/gen/isles0127_label_def.png}}; 
	\node at (\i+\shift+0.409*3, 0.95, 0.9*3) {\tiny $\phi \circ L$};
	}
 
	\foreach \i in {2.}
	{
	\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift-0.07*3,-0.17*3,-0.12*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.07*3,-0.17*3,-0.12*3) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.07*3,-0.17*3,-0.12*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;	
	\node at (\i+\shift-0.75, -0.35*3, -0.212*3) {\includegraphics[width=0.104\textwidth]{fig/gen/isles0127_patholprob_def.png}};
	\node at (\i+\shift-0.75, -1.64, -0.212*3) {\tiny $\phi \circ P$};
	}


	\node at (2.+1.04+\shift, 0.85, 0.25*3) {\includegraphics[width=0.1\textwidth]{fig/gen/gaussian.png}};
 
	\pgfmathsetmacro{\shift}{3.25}
 
	\node at (-1.0+1.15+\shift, -0.11, 0.25*3) {\tiny \text{Pathology-}};
	\node at (-1.0+1.09+\shift, -0.31, 0.25*3) {\tiny \text{enhanced}};
	\node at (-1.0+1.08+\shift, -0.51, 0.25*3) {\tiny \text{Sampling}};
	\node at (-1.0+1.05+\shift, -0.73, 0.25*3) {\tiny (\cref{eq: contrast})};
 
 
	\draw[-latex] (-1.15+0.6+\shift, 0.05, 0.25*3) -- (0.1+0.8+\shift, 0.05, 0.25*3);
	
	\draw[->, line width = 0.2mm, color=cb!90] (4.94+\dx+\shift, -2.63+\dy) -- (4.94+\dx+\shift, -2.87+\dy);
	\draw[->, line width = 0.2mm, color=matcha!150] (5.3+\dx+\shift, -2.63+\dy) -- (5.3+\dx+\shift, -2.87+\dy);
	\draw[->, line width = 0.2mm, color=tomato!70] (5.66+\dx+\shift, -2.63+\dy) -- (5.66+\dx+\shift, -2.87+\dy);

    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\pgfmathsetmacro{\dx}{0.} 
	\pgfmathsetmacro{\ddx}{-0.}
	\pgfmathsetmacro{\ddy}{-0.4}
        \foreach \dy in {4.}
        {
	\draw[dashed, color = flatgrey!80, line width=0.4mm] (4+\dx, -5+\dy+\ddy) -- (8.8+\dx+\ddx, -5+\dy+\ddy) -- (8.8+\dx+\ddx, -3.+\dy) -- (4+\dx, -3.+\dy) -- (4+\dx, -5+\dy+\ddy); 
        }
        
	\node at (1.5+1.66+\shift, 0.8+0.22, 0.25*3) {\tiny \text{w/ random Corruption $+$ Resampling}};
        
	\pgfmathsetmacro{\cubeza}{0.05*3}
	\pgfmathsetmacro{\cubezb}{0.02*3}
	\pgfmathsetmacro{\shift}{4.2}
	\foreach \i in {1}
	{
	\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift-0.1*3,0.*3,-0.1*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.1*3, 0.*3,-0.1*3) -- ++(0,0,-\cubezb) -- ++(0,-\cubey,0) -- ++(0,0,\cubezb) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.1*3,0.*3,-0.1*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubezb) -- ++(\cubex,0,0) -- cycle;
	
	\node at (\i+\shift-0.28*3, -0.18*3, -0.19*3) {\includegraphics[width=0.104\textwidth]{fig/gen/isles0127_sample_10.png}};
	\node at (\i+\shift+0.65, 0.23+1.3, 3.1) {\tiny $S_1$};
	}


	\pgfmathsetmacro{\cubeza}{0.03*3}
	\pgfmathsetmacro{\cubezb}{0.04*3}
	\pgfmathsetmacro{\shift}{4.2}
	\foreach \i in {2}
	{
	\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift-0.1*3,0.*3,-0.1*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.1*3, 0.*3,-0.1*3) -- ++(0,0,-\cubezb) -- ++(0,-\cubey,0) -- ++(0,0,\cubezb) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.1*3,0.*3,-0.1*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubezb) -- ++(\cubex,0,0) -- cycle;
	
	\node at (\i+\shift-0.28*3, -0.18*3, -0.19*3) {\includegraphics[width=0.104\textwidth]{fig/gen/isles0127_sample_4.png}};
	\node at (\i+\shift+0.65, 0.23+1.3, 3.1) {\tiny $S_2$};
 
	\draw[black,fill=black] (\i+\shift+0.36, 0.03, 0.25*3) circle (0.4pt);
	\draw[black,fill=black] (\i+\shift+0.46, 0.03, 0.25*3) circle (0.4pt);
	\draw[black,fill=black] (\i+\shift+0.56, 0.03, 0.25*3) circle (0.4pt);
	}
 
    \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=6ex},line width=1.pt,color = cb!80] (2+\shift-2.1, -0.0) -- (2+\shift+0., -0.0); 
	\node at (1.5+\shift+0.65, -0., 3.1) {\tiny T1w-resembled};
    
    \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=6ex},line width=1.pt,color = tomato!60] (2+\shift+.3, -0.0) -- (2+\shift+2.4, -0.0);
	\node at (4+\shift+0.53, -0., 3.1) {\tiny T2w/FLAIR-resembled};



	\pgfmathsetmacro{\cubeza}{0.05*3}
	\pgfmathsetmacro{\cubezb}{0.07*3}
	\pgfmathsetmacro{\shift}{4.2}
	\foreach \i in {3.5}
	{
	\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift-0.1*3,0.*3,-0.1*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.1*3, 0.*3,-0.1*3) -- ++(0,0,-\cubezb) -- ++(0,-\cubey,0) -- ++(0,0,\cubezb) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.1*3,0.*3,-0.1*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubezb) -- ++(\cubex,0,0) -- cycle;
	
	\node at (\i+\shift-0.28*3, -0.18*3, -0.19*3) {\includegraphics[width=0.104\textwidth]{fig/gen/isles0127_sample_14.png}};
	\node at (\i+\shift+0.65, 0.23+1.3, 3.1) {\tiny $S_{N-1}$};
	}
 


	\pgfmathsetmacro{\cubeza}{0.07*3}
	\pgfmathsetmacro{\cubezb}{0.04*3}
	\pgfmathsetmacro{\shift}{4.2}
	\foreach \i in {4.5}
	{
	
	\draw[black,fill=gray!30, line width = 0.02mm] (\i+\shift-0.1*3,0.*3,-0.1*3) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.1*3, 0.*3,-0.1*3) -- ++(0,0,-\cubezb) -- ++(0,-\cubey,0) -- ++(0,0,\cubezb) -- cycle;
	\draw[black,fill=gray!35, line width = 0.02mm] (\i+\shift-0.1*3,0.*3,-0.1*3) -- ++(-\cubex,0,0) -- ++(0,0,-\cubezb) -- ++(\cubex,0,0) -- cycle;
	
	\node at (\i+\shift-0.28*3, -0.18*3, -0.19*3) {\includegraphics[width=0.104\textwidth]{fig/gen/isles0127_sample_2.png}};
	\node at (\i+\shift+0.65, 0.23+1.3, 3.1) {\tiny $S_N$};
	}
	\end{tikzpicture}
	
}
\caption{
\texttt{UNA}'s on-the-fly generator uses 3D anatomy labels ($L$) and anomaly probabilities ($P$) to generate training data with diverse deformations, contrasts, and corruptions -- enhanced by varying intensity profiles in pathological regions.}
\label{fig: augment}
\end{figure}



